A Theoretical Approach for Structuring and Analysing Knowledge Provenance for Visual Analytics

The primary goal of Visual Analytics (VA) is to enable user-guided knowledge generation. Theoretical VA works to explain how the different aspects of a VA tool bring forth new insights through user interactivity, which itself can be captured through tracking methods for reproduction or evaluation. However, the process of automatically capturing the user's thought process, such as intent and insights, and associating it with user's interaction events are largely ignored. Also, two forms of interactivity capture are typically ambiguous and intermixed: the temporal aspect, which indicates sequences of events, and the atemporal aspect, which explains the workflow as sequences of states within a state-space. In this work, we propose Visual Analytics Knowledge Graph (VAKG), a conceptual framework that brings VA modeling theory to practice through a novel Set-Theory formalization of knowledge modeling. By extracting such a model from a VA tool, VAKG structures a 4-way temporal knowledge graph that describes user behavior and its associated knowledge gain process. Such knowledge graphs can be populated manually or automatically during user analysis sessions, which can then be analyzed using graph analysis methods. VAKG is demonstrated by modeling and collecting Tableau and visual text-mining workflows, where comparative user satisfaction, tool efficacy, and overall workflow shortcomings can be extracted from the knowledge graph.

==> TVCGDefinitions/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> TVCGDefinitions/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> eurovisDefinitions/EuroVisBody.tex <==
% ---------------------------------------------------------------------
% EG author guidelines plus sample file for EG publication using LaTeX2e input
% D.Fellner, v2.03, Dec 14, 2018


\title{From Data to Knowledge Graphs: A Multi-Layered Method to Model User's Visual Analytics Workflow for Analytical Purposes}

% for anonymous conference submission please enter your SUBMISSION ID
% instead of the author's name (and leave the affiliation blank) !!
% for final version: please provide your *own* ORCID in the brackets following \orcid; see https://orcid.org/ for more details.
\author[L. Christino \& F. V. Paulovich]
{\parbox{\textwidth}{\centering L.\, Christino\orcid{0000-0002-8754-8460}
        and F. V. Paulovich\orcid{0000-0002-2316-760X} 
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$Dalhousie University, Faculty of Computer Science, Canada
       }
}
}
% ------------------------------------------------------------------------

% if the Editors-in-Chief have given you the data, you may uncomment
% the following five lines and insert it here
%
% \volume{36}   % the volume in which the issue will be published;
% \issue{1}     % the issue number of the publication
% \pStartPage{1}      % set starting page


%-------------------------------------------------------------------------
\begin{document}

\teaser{
\vspace{-1cm}
 \includegraphics[width=\linewidth]{pictures/teaser.png}
 \centering
 \caption{Knowledge model unfolding for visual analytics. VAKG unfolds the interactions between the current knowledge model (A) into an interaction state-machine over time (B), which is then converted to a \textit{Temporal Knowledge Graph (TKG)} (C). Using set theory, VAKG can represent human knowledge generation and computer data mining and visualization as a structured TKG.
 }
 \label{fig:teaser}
}

\maketitle
%-------------------------------------------------------------------------
\begin{abstract}
% The importance of knowledge generation drives much of Visual Analytics (VA). User-tracking and behaviour graphs have shown the importance of understanding user's knowledge gain while performing VA workflows.
% % 
% We present VAKG, a theoretical framework which generalizes existing knowledge models and ontologies by focusing on how humans relate to computer processes temporally. 
% %
% For this, we propose an architectural model which structures this relationship as a 4-way Temporal Knowledge Graph (TKG) with specific emphasis in modeling the human and computer aspect of VA as separate but interconnected graphs.
% %
% Each lane provides a different dimension of the workflow: \textit{Interactivity} and \textit{Feedback} describes Knowledge Graphs (KGs) of immediately adjacent states of the computer workflow or of user behaviour States respectively, and \textit{Update Interface} and \textit{Knowledge} describes TKGs of the sequence of Updates of a given workflow and its users' knowledge gain respectively.
% %
% We propose that VAKG can define and generate a graph representing the temporal sequence of events and the relationship of states of the workflow in question, which are contained in the Update TKGs and State KGs respectively.
% %
% When considering multiple users' interactivity or multiple VA workflows, VAKG represents an overview of these workflows' usage and the collective knowledge generated by their users.
% %
% Although this structure is VAKG's basic contribution, it also expects other ontologies to expand its entity definitions, allowing the states and updates to be filled with data as property-maps or as interconnected sub-graphs.
% %
% We show that VAKG's structure allows for VA applications to use it as a provenance model, allowing for graph analytics of domain-specific processes, usage patterns, user's knowledge gain performance, among others.
%%
The importance of knowledge generation drives much of Visual Analytics (VA). User-tracking and behavior graphs have shown the importance of understanding users’ knowledge gain while performing VA workflows. We present VAKG, a theoretical framework that generalizes existing knowledge models and ontologies by focusing on how humans relate to computer processes temporally. We propose an architectural model that structures this relationship as a 4-way Temporal Knowledge Graph (TKG) with specific emphasis on modeling the human and computer aspect of VA as separate but interconnected graphs. VAKG can define and generate a graph representing the temporal sequence of events and the relationship of states of the workflow in question. When considering multiple users’ interactivity or multiple VA workflows, VAKG represents an overview of these workflows’ usage and the collective knowledge generated by their users. Although this structure is VAKG’s basic contribution, it also expects other ontologies to expand its entity definitions, allowing the states and updates to be filled with data as property-maps or as interconnected sub-graphs. We show that VAKG’s structure allows VA applications to use it as a provenance model, allowing for graph analytics of domain-specific processes, usage patterns, and users knowledge gain performance.

% This loosely coupled architecture aims to allow VAKG to be easily extensible and adaptable to a wide variety of situations and domains, including being extended to use other models or ontologies within itself. By using VAKG as a provenance architecture, the data gathered can also be easily used with existing graph analytics techniques, such as visualizations, shortest path analysis, recommendation systems, link prediction, temporal relationship analysis, and page-ranking.

% We present VAKG, a novel framework that defines a mathematical representation of the most known VA knowledge generation models and, with it, structures users' interactivity as a temporal Knowledge Graph. 
% %
% VAKG collects and links user interactivity, knowledge gain, and any other variable and structures them into temporal sequences of \textit{states} which are linked through \textit{updates}, resulting in a graph representation of the VA tool's usage (user interactivity) and the collective knowledge generated by its users. 
% %
% VAKG is a general-purpose data-structure framework that can be attached to any existing tool and can also be extended to adapt to a wide variety of situations and domains. 
\\
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
%   (see https://www.acm.org/publications/class-2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003145.10003147.10010365</concept_id>
<concept_desc>Human-centered computing~Visual analytics</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010178.10010187.10010193</concept_id>
<concept_desc>Computing methodologies~Temporal reasoning</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10002951.10002952.10002953.10010146.10010818</concept_id>
<concept_desc>Information systems~Network data models</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Visual analytics}
\ccsdesc[300]{Computing methodologies~Temporal reasoning}
\ccsdesc[100]{Information systems~Network data models}


\printccsdesc   
\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% START OF THE PAPER %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% The ``\maketitle'' command must be the first command after the
%% ``\begin{document}'' command. It prepares and prints the title block.

%% the only exception to this rule is the \firstsection command
\input{paper/main}

\bibliographystyle{EuroVisDefinitions/eg-alpha-doi}
%\bibliographystyle{plainnat}
% \bibliographystyle{abbrv}
% \bibliographystyle{abbrv-doi}
%\bibliographystyle{abbrv-doi-narrow}
%\bibliographystyle{abbrv-doi-hyperref}
%\bibliographystyle{abbrv-doi-hyperref-narrow}

\bibliography{references}
\end{document}

==> extra/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> paper/backup.tex <==


% To better understand the concept and applicability of \textit{knowledge}, significant research has been done by multiple areas beyond Visual Analytics. For instance, within \textit{Semantic Web}, the sub-areas of Knowledge Bases~\cite{TODO} and Knowledge Graphs~\cite{TODO} have shown many methods of how to interpret, store and query explicit knowledge, such as the information within wikipedia~\cite{todo dbpedia}. That said, the process of modeling data into a knowledge graph requires a well defined schema through ontologies, which is a common vocabulary to share information within a domain. 


% Techniques based on Graph-Theory also propose expansions on top of the current Knowledge Graph research. %??? TODO.. probably not
%%%

% compare to graph research area
% , including GNNs\footnote{GNN: Graph Neural Networks}~\cite{TODO}, graph visualizations~\cite{TODO} and graph operations~\cite{TODO}, such as page rank and traveling salesman, therefore many of the same algorithms and research are being utilized by both areas, creating a large potential for many future works within Visual Analytics.
%%%%

% Within VAKG, we have developed a concrete implementation of the VA loop as a concrete state-machine framework to be expanded upon.
% formalizing the flow of information within user-guided interactive tools.

% One possible categorization is to differentiate tacit knowledge, which is only in the mind of its owner, and explicit knowledge, which is able to be stored digitally and used to generate visualizations and analysis. \citet{sacha2014knowledge} thoroughly explains the differences and the applicability of tacit and explicit knowledge within VA, however how does the technical and domain knowledge needed by researchers to develop VA tools fits within this categorization?

%MAYBE CHANGE??% Finally, when considering all these aspects of knowledge, we can see that the development of Visual Analytics tools is considered to be a long and detail-oriented task~\cite{TODO}. Although Visual Analytics has been heavily used to analyse processes ranging from raw data analysis to machine learning model interpretation, the development of the tool itself is rarely analysed as a Visual Analytics problem, but mostly seen as a general software development task. For instance, when one wishes to develop a new VA tool, the technical aspect and the domain knowledge aspect within this development are often seen as separate entities, and only recently has become object of research~\cite{TODO}. Furthermore, the knowledge needed to build a VA system (e.g. technical and domain knowledge) and the knowledge treated in the VA system workflow itself are completely disconnected in the theoretical research and, consequently, in VA systems as a whole.



%% move to conclusion
% The general approach of software development utilizes metrics and analytics to gather, store and analyse the software in light of user usage, feedback and interactivity. Automatic systems like Google Analytics~\cite{TODO} has dominated both the market and the research platform as the tool of choice to collect user data to improve the existing software, perform A/B testing~\cite{TODO} and decide future goals for the product or research under development. Although the data collected through these means are valuable, it is not collected or analysed in the same light as the data used by the VA tool it monitors.

% ... The understanding of what knowledge is, how it is formed from the perspective of Data Analysis and Visual Analytics and the concept of how to model such knowledge generation into a shareable format is deeply discussed by \citet{collins2018guidance}. In their work, the author describes in detail what is intelligent guidance and how intelligent guidance, driven by insights from visualizations and results of machine learning applications, can provide digestible and interpretable information to users by reducing the cognitive load and bias that users may experience. Since user's analysis behaviour is dependent on their own pre-conceived knowledge and their own interest when starting an analysis process, \citet{collins2018guidance} also describes the model of user-knowledge and how visual analytics provides a method for users to generate and amass knowledge. In this context, the author describes knowledge graphs as an abstract representation of user-generated knowledge, which is contrasted by visual artifacts, such as annotations and bookmarks, which are considered to be explicit representation of knowledge.

% In our work, we will analyse knowledge graph concepts and publications when paired to its potential use within Visual Analytics with the same view as \citet{collins2018guidance}, where knowledge graph is both an abstract representation of user-generated knowledge and a graph-structured data model to store ontological interlinked concepts. Similarly, we will also analyse Dataspace's concepts and publications when paired to its use within Visual Analytics while focusing in its applicability in processing and organizing data. Our goal is to unify concepts of all three areas to propose potential research topics within Visual Analytics.


% \subsection{Learning Representations and Knowledge Graphs}\label{sec:knlowledgegraphs}
% As discussed previously, a Knowledge Graph~\cite{TODO} is a possible method of loosely linking the many heterogeneous datasets within a Dataspace. It is a concept originated from the Semantic Web~\cite{TODO} area and has been gaining traction as a graph representation of knowledge. In on itself, a Knowledge Graph, which is sometimes also called Knowledge Base, is a graph database where knowledge reasoning is modeled as connections between entities or properties. Connections like \"George Washington \textit{is a} human\" and \"Canada \textit{is a} country\" are examples of nodes connected by some reasoning. The process of modeling data into a knowledge graph requires a well defined schema through ontologies\footnote{a common vocabulary to share information within a domain}. 

% It is important to differentiate knowledge when in context of Visual Analytics, knowledge modeling, knowledge management, knowledge base, knowledge graph and ontologies. This differentiation will also be used to classify whether the surveyed publications utilized these concepts in their work. In simple terms:
% \begin{description}
%     \item[Knowledge,] in contrast to insight and information within the Visual Analytics context, is a structured, contextualized and generalized piece of information which can be understood and shared by its holder, such as "COVID-19 has caused lock-downs of most countries during 2020";
%     \item[Knowledge Base] is a digital dataset containing knowledge information which can be stored in a computer;
%     \item[Knowledge Graph] is a methodology to embed the knowledge base in a graph format. In one of its implementations, Resource Description Framework (RDF) expects that the knowledge is defined as multiple triples: two resources connected by a relationship;
%     \item[Ontology,] or Knowledge Modeling, is the architecture or schema of a given knowledge base. In RDF, for example, ontology relates to what is the definition of an resources and of a relationship within the knowledge base's domain and context. See DBPedia~\cite{TODO} for a specific example;
% \end{description}
% %TODO: differentiate between knowledge base and knowledge graph.. talk about this in the next few sections and include "The Role of Explicit Knowledge: A Conceptual Model of Knowledge-Assisted Visual Analytics" as a reference

% The main open-source example of knowledge graphs is DBPedia~\cite{TODO}, where all information of Wikipedia is segmented into well defined ontologies for simple queryable operations. \citet{chen2020review} segments the usage of Knowledge Graphs into three categories: rule-based reasoning, distributed representation-based reasoning and neural network-based reasoning. Applications of knowledge graphs can be extended to recommender systems, health systems, fintech and question-answering systems, all of which is discussed by \citet{chen2020review}.

% Of course, knowledge graphs has many parallels and connections to the overall graph research, including GNNs\footnote{GNN: Graph Neural Networks}~\cite{TODO}, graph visualizations~\cite{TODO} and graph operations~\cite{TODO}, such as page rank and traveling salesman, therefore many of the same algorithms and research are being utilized by both areas, creating a large potential for many future works within Visual Analytics.


% We will analyse and categorize the most cited research found in Visual Analytics which involves the usage of knowledge bases, graph theory, dataspaces and visual analytics concepts. Similarly, we will also categorize them as by their objective type in an attempt to show any bias towards specific objectives as well as gaps of potential research objectives when considering the classification of each area described previously.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% By analysing existing works in visual analytics, especially ones which define possible framework-level methodologies to develop visual analytics applications~\cite{wang2016survey}, we are able to define our method for survey and review of existing Knowledge Graph research in light of the Visual Analytics framework. In summary, Visual Analytics represents a framework which unifies concepts of the data-domain, visualization domain, analysis domain and human-computer-interaction domain. This sub-division will be important for our study, therefore to be more specific:
% \begin{itemize}
%     \item Data: All data characteristics will be treated as either a Dataspace concept, such as pre-processing, or Knowledge Graph concept, such as data schema. See Sec.\ref{sec:dataspaces} and Sec.~\ref{sec:knlowledgegraphs};
%     \item Analysis:
%     \begin{description}
%         \item[Analysis of focus] Before developing a Visual Analytics application, the developer must decide what type and format of analysis is expected to be done with it. Examples are Exploratory Data Analysis~\cite{TODO}, Confirmatory Analysis~\cite{TODO}, Descriptive Analysis~\cite{TODO}, Predictive Analysis~\cite{TODO}, among others;
%         \item[Visual Analysis Modeling] With both the analysis type and data in mind, the developer is then responsible to model an analysis workflow and transform it into interactive visualizations;
%         \item[Iterative Analysis] VA tools have increasingly utilized an iterative methodology to aggregate knowledge~\cite{TODO}, especially though the use of Active Learning~\cite{TODO};
%     \end{description}
%     \item Visualization and Interface:
%     \begin{description}
%         \item[Visualization Type and Number] Simple count of the number and types of visualization used within~\cite{TODO};
%         \item[Dashboard Workflow] In light of the analysis workflow developed, the dashboard is designed to promote this workflow in the best manner possible;
%         \item[AI Explanation] We have seen a great increase of efforts to explain machine learning models' decisions and inner-workings to users through visualizations;
%     \end{description}
%     \item Information and User-Knowledge:
%     \begin{description}
%         \item[Finding Generation and action~\cite{TODO}] user's first level of gathering information from the application and acting with it for further analysis, usually focused in Exploratory Analysis~\cite{TODO};
%         \item[Insight and Hypothesis Confirmation~\cite{TODO}] user upgrades his finding into an insight by observing and absorbing more information from the tool, and transforms into an hypothesis through statistics testing or other similar methods, usually focused in Confirmatory Analysis;
%         \item[Knowledge~\cite{TODO}] our main focus in the study, since it is the core intersection with Knowledge Graphs;
%         \item[Manual versus Automatic Knowledge] Machine learning also affects how Visual Analytics tools are developed, since some expect users to gather information~\cite{TODO} and others generates the information either beforehand~\cite{TODO} or at the instant~\cite{TODO} when users interact with the application;
%     \end{description}
% \end{itemize}

% Our survey will utilize these definitions and partitioning of the visual analytics framework to classify existing publications into weather they can be considered a Visual Analytics project or, even more important for our research, what are the potential benefits of utilizing Knowledge Graphs and Dataspaces to improve results.
%%%%%%%%%%%%%%%%%%%%%%%

Seen all these concepts of Knowledge Graphs and Visual Analytics, \citet{chang2009defining}, \citet{chen2019ontological} and \citet{sacha2018vis4ml} thoroughly discusses many aspects and intersections between Knowledge Bases and Visual Analytics. In summary, Visual Analytics attempt to provide a workflow for knowledge generation through the use of relevant data mining processes and interactive visualizations~\cite{wang2016survey}, and Knowledge Graphs provide a format and methodology of knowledge storage, retrieval and extensive mechanisms to for knowledge embedding. This very simplistic view of the fields already clearly outlines intersections to be explored such as knowledge modeling, where knowledge base research cab provide a platform for Visual Analytics tools to record user-generated knowledge for posterior use, and visualization insights. For instance, Vis4ML~\cite{sacha2018vis4ml}'s core proposal uses a framework based on Knowledge Graphs to describe Visual Analytics usage throughout the Machine Learning research area. Applications such as analysis recommendations~\cite{burke2000knowledge, wang2018ripplenet}, CSCW~\cite{chang2009defining} and automatic knowledge extraction through active learning~\cite{TODO} have also demonstrates how to intersect Knowledge Graphs and Visual Analytics.

Many recent research publications explicitly utilizes knowledge graphs within Visual Analytics. CAVA~\cite{cashman2020cava} is the most recent, in which users gather more insights by utilizing DBPedia Knowledge Graph's ontologies to augment the existing data during analysis, such as joining countries' GDP per capita from DPBedia into the existing data. This is done interactively while the user performs exploratory analysis of their data or while they select features to be used in the training process of machine learning models. CAVA's strict usage is for augmenting existing data with DBPedia while exposing the newly formed data to external tools, such as Tableau for actual analysis. Therefore CAVA is not attempting to manage many heterogeneous datasets as discussed in the dataspace section, nor utilizing AI or graph theory to utilize Knowledge Graphs in its fullest, but only unite two datasets, namely an existing tabular data and DPBedia, in an attempt to augment visual analytics tasks.

Another recent work is Google's work on visualizing and analysing mobile apps through Knowledge Graphs~\cite{chang2016appgrouper} called AppGrouper. It uses a human-in-the-loop interactive tool for app clustering utilizing a knowledge-graph-based clustering process, where the authors argue that the algorithmic-only machine learning procedure previously used could learn from this work. Although this work is very innovative while utilizing large datasets, human-in-the-loop process, \"pay-as-you-go\" mentality when constructing data and knowledge and good advances on Knowledge Graph's machine learning applications, it lacks the visual component found in visual analytics and the data framework utilized is not open for additional heterogeneous data as dataspaces are intended to be. Nonetheless, much is learned applied from this work, including ConceptVector~\cite{park2017conceptvector}, which is a proper visual analytics tool to analyse text through a human-guided lexicon builder. \citet{park2017conceptvector} argues that ConceptVector is able to better allow text analysis than the state-of-the-art due to its human-in-the-loop component of defining words of interest in order for it to automatically build a knowledge-graph-based word embedding to, finally, provide and correlate the specific textual concepts from a text database. However, ConceptVector does not actually uses Knowledge Graphs and is limited by a single textual dataset as the focus of analysis.

% TODO: review if it uses knowldege base or knowledge graph
\citet{chen2018viseq} and \citet{sacha2016analytic} on the other hand focuses on the generation of a Knowledge Graph which does not match Knowledge Graph research. \citet{sacha2016analytic}'s main objective is to provide ways for users to initiate an analysis and record their findings with bookmarks and annotations during analysis, and with the resulting Knowledge Graph users are able to validate if they confirmed their previous assumptions or not. Although this is an interesting way of generating trust in user's analysis and results, the system merely generates a graph with the generated knowledge, but does not follow any of the research done in Knowledge Graphs themselves, do not provide autonomous or intelligent mechanisms within its Visual Analytics portion and focuses on analysis and not on the data, which moves it away from dataspace research. Similarly, Viseq~\cite{chen2018viseq} provides a way to visualize online courses sequences for better learning, however this was mostly an application of a graph-like structure and visualization without any Knowledge Graph research to back it up.

An older work by \citet{chang2009defining} went through great lengths to develop a knowledge-assisted Visual Analytics tool, where their dataset is tightly integrated with a graph dataset of expert's knowledge. This data structure and the tool's interactive components provided their users with great CSCW applicability. Although they had a great introductory description, their tool does not utilizes the full potential of the current research of machine learning within Knowledge Base and Visual Analytics, and similar to most of the previous works, there is no attempt to utilize dataspaces concepts. Their own limitation discussions adds to the limitation of their Knowledge Base implementation and lack of data integration procedures to avoid duplicates within it or, better yet, to utilize these duplicates as reinforcement of knowledge to provide a more intelligent analysis.

%likely move upwards the next paragraph
As thoroughly discussed and exemplified by \citet{federico2017role}, Visual Analytics utilizes heavily the term and concept of knowledge and knowledge modeling when considering what users learn from both visual and interactions with a Visual Analytics tool. (talk about the works within TODO). However, as was discussed before at Sec.~\ref{TODO}, knowledge graphs is the central point of our survey due to its linking property. Therefore, all works discussed and knowledge models themselves~\cite{federico2017role} do not handle linking heterogeneous datasets, merely treating data as a concise and unified entity (TODO: maybe include figures from them). Furthermore, the graph-structure present in knowledge graphs provides the benefits of modeling and embedding knowledge into machine learning models, provide direct visualization potentials and allows for graph-specific operations to be analysed and utilized by the Visual Analytics community, such as knowledge page-rank, recommendations and construction/pattern analysis, all of which is not tackled neither by \cite{federico2017role} nor by any other work we have surveyed.


When also considering Dataspaces, further connections and potential areas of intersections emerge. As was discussed in Sec.~\ref{sec:dataspaces}, dataspaces tackle the issue of storing and linking multiple heterogeneous datasets in a \"pay-as-you-go\" manner. These links can be defined as a type of meta-knowledge about the datasets in question, and can be stored in a graph structure~\cite{chen2020review}, among other possible structures. Similarly, both the datasets themselves and their links are expected to be open for analysis and exploration, which are also shared with concepts from Visual Analytics.
----TODO: write more and get info from below sections to put here ---

\paragraph{Data Integration}
Data integration is another vast research field which has had several publications in method to integrate heterogeneous datasets, however usage within dataspaces will be the focus of our survey, therefore the methods described in Sec.~\ref{sec:dataspaces} of entity matching~\cite{TODO}, entity resolution~\cite{TODO}, entity deduplication~\cite{TODO} and semantic resolution~\cite{TODO} will be the techniques analysed within our survey. Although these methods and techniques have all had publications with visualization aspects~\cite{TODO}, they have caught our attention due to not have been thoroughly investigated within Visual Analytics publications~\cite{kopcke2010frameworks}. For example, the DDupe system and its applications~\cite{kang2008interactive, bilgic2006d} demonstrate a certain usage of entity matching concepts within Visual Analytics, but always focusing its analysis within a restricted dataset.

Many other concepts and areas of research, such as databases, networking, multi-dataset machine learning, time-series machine learning, graph-neural-networks, and so on, however we will limit our survey to the broad intersection of the three areas while describing these specific potential use-cases at the end.

\begin{itemize}
    \item 
\end{itemize}

Following the description of visual analytics pipeline done by~\citet{wang2016survey}.

\begin{table}[tb]
\caption{VIS/VisWeek accepted/presented papers: 1990--2015.}
\label{tab:papers}
\scriptsize
    \centering
\begin{tabularx}{\columnwidth} { | X | X | X | }
     \hline
     item 11 & item 12 & item 13 \\
     \hline
     item 21  & item 22  & item 23  \\
    \hline
\end{tabularx}
\end{table}

\section{Potential Research Opportunities}
We can see that most of the research done so far either do not fully utilize the background and research of all areas or, in some cases, even misuse the terms. Our main motivation of producing this survey was because we observed these issues consistently while also foreseeing great advantages and many potential future work for all areas involved to utilize deeper concepts and research of each other. In this section we will list and analyse potential opportunities for research in Visual Analytics when considering the classifications and limitations of the publications of Table~\ref{tab:papers}.


\subsection{Data Storage, Retrieval and Linking}

Within big data, it is hard to expect users to properly be able to fully utilize and link all data provided to them in a tool. Works like \cite{song2019big, li2020marrying} attempts to provide a way to utilize Knowledge Graphs as a storage layer to retain information gathered during an exploratory analysis session. Then, the Knowledge Graph can be used to organise and provide valuable insights to users given previous user's insights and other automated data mining algorithms, such as clustering and association analysis. \citet{song2019big} in specific utilizes the relationship between products of the same category to generate a visual-guided tool for risk analysis, and \citet{li2020marrying} stores previous exploratory analysis to further use in Machine Learning processes.

Other tools utilize existing Knowledge Graphs to either explore their content or enhance an external dataset. Works like \cite{song2019big, chen2020review} investigates the twitter and Wikipedia knowledge graphs respectively in an attempt to make sense and bring forth latent insights stored within.

\paragraph{Graph Databases}
Knowledge Graphs systems utilizes graph-specific databases to store data. Most systems use either are Neo4J~\cite{TODO} or AWS Neptune~\cite{TODO}, but there are many more options~\footnote{A list of graph databases can be seen at \url{https://www.g2.com/categories/graph-databases}}. However, of the Visual Analytics and Dataspaces research discussed so far, only a few use Neo4J, and its use is restricted to storing the data. Research in these areas have yet to utilize these technologies as the research focus. Opportunities lie in ideas such as visualisation of Neo4j inner workings and optimizations, use of graph databases as the linking mechanism within dataspaces and, of course, a visual analytics system to explore these linked dataspaces.

\subsubsection{Data Integration}\label{sec:dataintegration}
As is discussed in Sec.~\ref{sec:dataspaces}, data integration is another large research field which has had several publications in method to integrate heterogeneous datasets within dataspaces~\cite{TODO}. Here we will discuss some potential research opportunities to Visual Analytics.

\paragraph{Entity Resolution}
~\cite{kang2008interactive, moreauvisual} example~\cite{bilgic2006d}

\paragraph{Entity Deduplication}
~\cite{muelder2016visual, morton2016view}

\paragraph{Semantic Resolution}

\subsection{Machine Learning}
Application such as \cite{li2020marrying} applies Knowledge Graphs to retain knowledge from external datasets and applies it into Graph-based Neural Networks models. \citet{li2020marrying} in specific uses an attention-based approach, approximating Knowledge Graphs to the state-of-the-art NLP\footnote{NLP: Natural Language Processing} ML frameworks, such as BERT~\cite{TODO} and GPT-3~\cite{TODO}.

\paragraph{Graph Neural Network}
Visual Analytics has only recently been in contact with GNNs~\cite{jin2020gnnvis}, but many other opportunities lie ahead. For instance, Knowledge Graphs are a graph-based structure, therefore the Knowledge Graph research group has heavily utilized graph-based machine learning techniques, such as GNNs, applied to many different aspects of knowledge, knowledge modeling and automatic knowledge generation. Visual Analytics seems to be a natural next step to bring intelligent knowledge graphs to users by using both GNNs and visualizations to provide value.

\paragraph{Time-Series Machine Learning for Real-Time Datasets}
Realtime-linked dataspaces~\cite{curry2020real} show how a data retrieval and storage system can be used to not just hold IoT data but also use stream-based processes to process the data into a usable format, similar to what is done with static datasets within Visual Analytics. Although several applications of realtime data are used within Visual Analytics~\cite{TODO}, they don't treat the data as a complex interlinked dataspace, but only as a single dataset. An example is the lack of real-time Visual Analytic systems for autonomous vehicles, where the few existing projects don't treat the data as real-time~\cite{gou2020vatld, wangvvisual}. Therefore, the applicability of time-based machine learning~\cite{} and other real-time and streaming processes which require multiple linked datasets aren't used or researched within Visual Analytics as of yet.

\paragraph{Active Learning}\label{p:activelearning}
Within active learning research, we find that most of the current projects are done in-situ~\cite{TODO}, where the generated labeled-data from the active learning process is held by the system itself in one way or another. Even though the growth over time of active learning systems are strongly related to dataspaces, the accumulated knowledge is not integrated with the data pipeline of Sec.~\ref{sec:dataspaces}. Many potential research opportunities lie on integrating and sharing accumulated knowledge back to the open dataspace of the Web. Adjacently, this newly generated labeled-data is mostly used for supervised, semi-supervised or reinforcement learning optimizations, and not treated as knowledge. Therefore, other research opportunities lie in the usage of the generated data as extensible knowledge within a knowledge base or knowledge graph, from where the techniques discussed in Sec.~\ref{sec:knlowledgegraphs} can be applied.

\subsection{Visualization}
Visualization is one of the cornerstones of Visual Analytics. In this section we investigate and discuss potential research opportunities of new visualizations to be developed.

\paragraph{Graph Visualizations}
Although we don't claim to have surveyed the graph visualization research area, another potential research direction we have found through our survey is the usage of modern and state-of-the-art methodologies of graph visualization, including techniques of dimensionality reduction and projection, Virtual Reality and other similar research. Visual Analytics' attempt to visualize Knowledge Graphs focuses on the simple linked-bubble chart as seen in Sec.~\ref{sec:overview}, however more visual embedding and interactive elements could be explored for both the visualization and the manipulation of Knowledge Graphs and of the links between datasets within a dataspace, where concepts of Active Learning (P.~\ref{p:activelearning}) and Data Integration (Sec.~\ref{sec:dataintegration}) can be applied.

\paragraph{Dataspace Links}
Visual Analytics and Dataspaces shares many of the data processing and data mining. However, the visualization of dataspaces is in its infancy, and the use of the entire Visual Analytics' framework of interactive analysis and manipulation of data is yet to be seen within the Dataspace research area. Visual Analytics has publications utilizing multiple linked datasets~\cite{TODO}, but as was discussed it also has yet to utilize an actual dataspace implementation. Therefore Further opportunities lie in the research and development of Dataspace systems which uses Visual Analytics for ongoing addition of new data and links between data stored within.

\paragraph{Cartographic Visualization}
The cartography method of encoding visual information are also of great benefit for to Visual Analytics research when considering how to improve the visualization and interactivity of Knowledge Graphs and Dataspaces. For example, \citet{viegas2004social} proposes mother ways of visualizing graphs in light of cartography, and similar concepts could be applied for Visual Analytics' visualization of Knowledge Graphs and Dataspaces.

\paragraph{Interactivity and User Feedback}
Visual Analytics largely exploits interactive visualizations to provide user-guided analysis. Dataspace's pay-as-you-go concept and knowledge graph's query systems, such as DBPedia, proposes a similar thread where user-guided interaction with the systems provide an enhanced experience for each of the use-cases. Unfortunately these three similarities have not been used in conjunction as of yet. Examples of the use of Visual Analytic's interactivity to perform Knowledge Graph visualizations and visual query exists~\cite{he2019aloha}, but they are largely contained within a single secured dataset and with the sole focus on analysing the existing data rather than enhancing and adding to the Knowledge Graph new data collected from the user. The use of Visual Analytics framework methodology~\cite{wang2016survey} and exploratory patterns done by users~\cite{} can be utilized to append new knowledge gathered through direct means, such as user-generated annotations, and indirect means, such as through user's natural use of the tool.

\section{Conclusion}

One of the limitations within the research of dataspaces is that there is little to no publications tackling visualization or visual analysis of the dataspace itself, instead focusing on the framework methodology itself and the monitoring of the entities contained within. We argue that many strong future work relies on creation of visualizations and visual analytics tools specific for the overall monitoring, control and analysis of dataspaces as a whole.


==> paper/bck_interviews.tex <==
% \section{VAKG in Practice: Interviews for Potential Applications}\label{sec:interview} %revisar

% During the development of VAKG, Janio was kind enough to give inputs related to the usefulness of tracking user interactivity for knowledge gain. Janio is an experienced entrepreneur and business owner in the international food supply chain as an international food importer and wholesaler, and regional restaurant chain ownership and management with over 30 years of experience. The hour-long interview focused on his methods to store information and extract knowledge from Enterprise Resource Planning (ERP) and Accounting systems. In summary, he said the usual process depends heavily on training employees to record sales manually and restocking data in a system. Once the data is stored and structured into a timeline of events, he generates reports and uses his own business experience to discover and explain insights from the data. We have included a small excerpt of the interview below.

% \textit{Q: Can you give examples of when and how you use provenance and analysis?} 
% %
% One example is how I analyze the product purchase behavior of select customers on a month-to-month basis and the overall monthly product-based sales compared to previous years. I do this by extracting all reports from my accounting software and using MS Excel to merge them and analyze the result, sometimes on a month-by-month basis or a year-over-year basis, depending on what I am analyzing. (...) Among the main difficulties within the process is the required expectation of correct imputation by the employees and the amount of external knowledge I need to bring to the report so that analysis can be meaningful. In our restaurants, employees would input the payment type of a purchase, such as cash or credit card. However, once the customer makes the payment, sometimes the type would swap, but the system is not updated, causing many discrepancies in the monthly accounting process.

% \textit{Q: How external knowledge was used and was it included in the reports?} 
% %
% (...) managers typed in manually certain events, such as heavy rain or large soccer match, while inputting the weekly restocking information. (...) however, most of the time, the external knowledge I use is either only manually typed during the analysis itself after the generated report or not included at all, just coming from my head, experience, and the internet.

% %\subsection{Data Scientist Interview.} 
% We also interviewed Thiago, a Data Science General Manager of Credit Recovery in a large bank. Thiago has a Ph.D. in Machine Learning applied to Natural Language Processing and has over a decade of industry experience in applied data science. In summary, we discussed in his interview the past and present use of provenance analysis within decision-making processes.

% \textit{Q: Can you give examples of when and how you use provenance and analysis?} 
% %
% Bank transaction provenance, such as payments and money transfers, is extensively used for flagging fraudulent transactions. (...) My area then uses machine learning to predict the tendency of credit repayment. The treatment of temporal relationships of the data, such as order of transactions, is sometimes part of an embedding step or forwarded to a machine learning model which can handle temporal data. A new project in my area uses provenance to better design a data science workflow. Currently, our bank does not have a well-optimized data analysis workflow. Still, by tracking the data analysis, we plan to record the work effort of each task and, in the future, analyze the results to improve the overall workflow or help us plan the future by predicting how long data analysis tasks will take.

% \textit{Q: Would a temporal knowledge graph structure, such as the one from VAKG, aid in such applications? How? } 
% %
% A co-worker and I have been investigating using a knowledge graph representation of customers that could describe behavioral patterns for better predictions during fraud analysis. (...) Another large intersection I see is by using such a structure to record and analyze our Data Science pipeline. Using such recording, we envision predicting a more optimized sequence of tasks required for a new data science project given a description of goals or problems we want to solve.

% We use these interviews to check in the wild the significance of our motivation, goals and get insights into future works for VAKG when applied to real business analytical processes. For instance, Janio confirmed that his experience with ERP and accounting software essentially had data provenance but rarely tracked any external information at the time when the data was changed, such as the reasoning of why his employee changed the data (\textbf{G1}). Janio said he manually had to track down these extra pieces of information through an involved and time-consuming cross-check process and use external software to merge and analyze it (\textbf{G2} \& \textbf{G3}).

% Similarly, Thiago's usage of provenance requires significant work by data scientists for analysis to process the data (\textbf{G2} \& \textbf{G3}), and his wish to better understand this data science pipeline through provenance and knowledge graphs indicates both the lack and the potential of using VAKG (\textbf{G1}). These examples show that VAKG's focus on tracking the user's knowledge gain in tandem with user interactivity aims to aid in this problem: the analysis of data-oriented workflows that requires or would benefit from the connection between data provenance, external data (e.g., supply chain or bank transactions) and user knowledge gain (e.g., intentions and behavior). 


==> paper/tomove.tex <==
%Subsequent theoretical advances were proposed~\cite{federico2017role}, showing that the framework of knowledge generation flow is not consistent throughout the VA research, but even so, the importance of knowledge generation continues to drive much of the state-of-the-art tool development within VA. 
%



%  General outline of VAKG's graph structure. 
%  .A VA tool [A] called ExPatt used VAKG to track its interface states and user's knowledge gain [B]. The tool's state [C] is stored as a property map, including metadata and links to external data, and on each update operation (e.g. an interaction on the tool) a new update node [D] records all pertained information, including timestamp and user id. Similarly the user's ongoing insights and tacit knowledge follows the same structure in a separate graph [E,F]. Overall, VAKG links the user's interactions on the tool to their knowledge gathering process [G], providing access to graph-based relationship and path analysis, such as page-rank, recommendations and path prediction in addition to a concrete framework for developers to follow in order to apply the VA knowledge loop methodology of \citet{sacha2014knowledge}


% Such a concrete framework would allow researchers to both optimize the development time and provide knowledge-related enhanced capabilities to every tool while also being confident that their tool follows the VA's theoretical framework of knowledge flow. However, we have not seen as of yet any attempt to put this into practice.
%
%FVP: aqui ainda estamos na motivacao, entao nao faz muito sentido discutir solucao. Tem que passar essa setenca abaixo para o lugar onde discutimos solucao. 
% 
%Through VAKG we attempt to fill this gap by systematizing the theoretical Visual Analytics knowledge flow as a concrete mathematical framework and, from that, providing a sample implementation of a system which provide the required functionalities. Therefore, VAKG provides a general-purpose data-structure framework which can attach to other existing technologies or tools in either a system architecture, an online service interface or as a library module.
